Simulating systematic bias in attributed social networks and its effect on rankings of minority nodes

Network analysis provides powerful tools to learn about a variety of social systems. However, most analyses implicitly assume that the considered relational data is error-free, reliable and accurately reflects the system to be analysed. Especially if the network consists of multiple groups, this assumption conflicts with a range of systematic biases, measurement errors and other inaccuracies that are well documented in the literature. To investigate the effects of such errors we introduce a framework for simulating systematic bias in attributed networks. Our framework enables us to model erroneous edge observations that are driven by external node attributes or errors arising from the (hidden) network structure itself. We exemplify how systematic inaccuracies distort conclusions drawn from network analyses on the network analysis task of minority representations in degree-based rankings. By analysing synthetic and real networks with varying homophily levels and group sizes, we find that introducing systematic edge errors can result both in a strongly increased or decreased ranking of the minority. The observed effect depends both on the type of edge error considered and level of homophily in the system. We thus conclude that the implications of systematic bias in edge data depend on an interplay between network topology and type of systematic error. This emphasises the need for an error model framework as developed here, which provides a first step towards studying the effects of systematic edge-uncertainty for various network analysis tasks.

==> Results_Copenhagen.tex <==
\begin{comment}
Our analysis of both synthetic and real-world networks emphasise that the robustness of network analysis results with regard to a specific bias depend on the particular network topology.
Hence, we have to examine the particular network data of interest in detail under specific noise hypothesis, which we can simulate with our model.
In this section, we illustrate this by applying our model to different communication and interaction channels of a social network. 
Each of these channels may be seen of providing a different, potentially biased view on the underlying latent social network.
In particular, we use the different interaction networks which were collected via smartphones as part of the Copenhagen Network Study \cite{sapiezynski_interaction_2019}. 
We include the network of physical proximity among the participants (estimated via Bluetooth signal strength), the network of phone calls, the network of text messages, and the network of Facebook friendships. 
A summary of the network statistics can be found in Table \ref{tab:copenhagen}.

\begin{table}[b]
\caption{\textit{Overview of Copenhagen Network Study networks} \cite{sapiezynski_interaction_2019}. { As in Table \ref{tab:real_data}, we use $Q_{mod}$/$A$ to denote the modularity/assortativity of the partition based on minority and majority label. Both metrics may be interpreted as a proxy for the homophily in the dataset. The fraction of the minority in the dataset is denoted by $f$.}
    }
\small 
    \centering
\begin{tabular}{l | r rrr r}
                 name &  nodes &  edges & $Q_{mod}$ &  $A$ &             $f$ \\
\midrule
  Facebook &    744 &   5865 &    0.043 &       0.11 &  22\% \\
   Sms &    429 &    580 &    0.093 &       0.23 &   27\% \\
   Calls &    322 &    440 &    0.081 &       0.22 &   25\% \\
    Bluetooth (Face-to-face) &    658 &  74808 &    0.01 &       0.03 &  22\% \\
\end{tabular}
\label{tab:copenhagen}
\end{table}

\subheader{Motivation}
People have diverse interests and preferences for communication
and they show different usage patterns of services. Therefore, certain groups of people may prefer specific communication channels. This influences the shape of the social network captured by the the different service channels. The network of people who call each other may thus be different to peoples' real-world interactions. For example, women might tend to use phone calls as mode of communication more often than men. An individual's choice of communication channel can therefore be seen as a sampling procedure driven by context factors and bias \cite{torok_what_2016}. 

\subheader{Modeling bias hypotheses}
With our model, we can capture the effects of different kinds of systematic bias which influence a person's choice of communication channel. In particular, we look at face-to-face interactions, phone calls, text messages and Facebook friendships in the Copenhagen Network Study. Our error model allows to simulate all variations of biases in the different layers of the data set in order to check the robustness of the derived rankings. For example, the previous example of systematic gender differences in phone calls would result in a group specific minority bias. We provide a complete overview of simulations for all node attribute-based and structure-based biases in Figure \ref{fig:copenhagen_labelnoise} and \ref{fig:copenhagen_edgenoise}.

\subheader{Implications}
The simulations show, that in these communication networks the minority representation in node-degree based rankings are robust with regard to all kinds of \emph{structure-based} noise for all communication channels. We may thus conclude that results of rankings are likely not much affected by biases that are captured by this type. 

In contrast, all simulated \emph{attribute-based} noise types show strong effects on the ranking results. This may indicate that bias that is based on group membership of nodes, which represents systematic gender differences in this case, has high impact on minority representation in rankings based on communication networks.

\begin{figure*}[ht]
	\begin{center}
	\begin{subfigure}[c]{2.0\columnwidth}
				\includegraphics[width=\textwidth]{figures/legend10.pdf}
		\end{subfigure}
		\begin{subfigure}[b]{0.386847\columnwidth}
			\includegraphics[width=\textwidth]{figures/real_retain_copenhagen_bt.pdf}
			\caption{Face-to-face}
		\end{subfigure}
		\begin{subfigure}[b]{0.452612\columnwidth}
			\includegraphics[width=\textwidth]{figures/real_retain_copenhagen_facebook.pdf}
			\caption{Facebook}
		\end{subfigure}
		\begin{subfigure}[b]{0.386847\columnwidth}
			\includegraphics[width=\textwidth]{figures/real_retain_copenhagen_calls.pdf}
			\caption{Calls}
		\end{subfigure}
		\begin{subfigure}[b]{0.386847\columnwidth}
			\includegraphics[width=\textwidth]{figures/real_retain_copenhagen_sms.pdf}
			\caption{SMS}
		\end{subfigure}
	\end{center}
\caption{\textit{Effect of node attribute-based noise on Copenhagen dataset}. {Similar to Fig.~\ref{fig:retain} we plot the influence of the retain parameter $\rho$ on the different communication channels of the Copenhagen Network dataset. From left to right the networks show increasingly higher modularity which can be  seen as a proxy for homophily, if the connectivity of the network is indeed driven by homophily. The effects of the different noise types are present in all communication channels.}}
\label{fig:copenhagen_labelnoise}
\end{figure*}


\begin{figure*}[ht]
	\begin{center}
	\begin{subfigure}[c]{2.0\columnwidth}
				\includegraphics[width=\textwidth]{figures/legend_struct10.pdf}
		\end{subfigure}
		\begin{subfigure}[b]{0.386847\columnwidth}
			\includegraphics[width=\textwidth]{figures/real_retain_alpha_copenhagen_bt.pdf}
			\caption{Face-to-face}
		\end{subfigure}
		\begin{subfigure}[b]{0.452612\columnwidth}
			\includegraphics[width=\textwidth]{figures/real_retain_alpha_copenhagen_facebook.pdf}
			\caption{Facebook}
		\end{subfigure}
		\begin{subfigure}[b]{0.386847\columnwidth}
			\includegraphics[width=\textwidth]{figures/real_retain_alpha_copenhagen_calls.pdf}
			\caption{Calls}
		\end{subfigure}
		\begin{subfigure}[b]{0.386847\columnwidth}
			\includegraphics[width=\textwidth]{figures/real_retain_alpha_copenhagen_sms.pdf}
			\caption{SMS}
		\end{subfigure}
	\end{center}
\caption{\textit{Effect of structure-based noise on Copenhagen dataset.} In analogy to Fig.~\ref{fig:retain2} we show the impact of structure-based noise. 
Overall we can see that structure-based noise does show strong effects on the minority representation in rankings based on the communication channels of the Copenhagen dataset.}
\label{fig:copenhagen_edgenoise}
\end{figure*}

\end{comment}
